Deep Physiological State Space Model for Clinical Forecasting

Clinical forecasting based on electronic medical records (EMR) can uncover the temporal correlations between patients' conditions and outcomes from sequences of longitudinal clinical measurements. In this work, we propose an intervention-augmented deep state space generative model to capture the interactions among clinical measurements and interventions by explicitly modeling the dynamics of patients' latent states. Based on this model, we are able to make a joint prediction of the trajectories of future observations and interventions. Empirical evaluations show that our proposed model compares favorably to several state-of-the-art methods on real EMR data.

==> append.tex <==
\section{Model Selection}



LSTM-based solutions use a hidden state size of $20$ and learning rate of $0.00075$ and $DSSM$ uses a hidden state size of $30$ and learning rate of $0.0001$. In the experiment, each timestep take $1$ hour, and the prediction rolls out to $120$ hours for both state-based hazard rate models. 
 
 
 
\section{Dataset Statistics}


  \begin{longtabu}{p{1cm}p{6cm}XXX}\caption{List of input features used in the model.} \label{tab:features} \\ \toprule
Index&
Observation Name&
LOINC code&
MIMIC specific code&
Units\\\midrule
\endhead
\bottomrule
\endfoot
0&
Heart Rate&
&
211&
bpm\\
1&
SpO2&
&
646&
percent\\
2&
Respiratory Rate&
&
618&
bpm\\
3&
Heart Rate&
&
220045&
bpm\\
4&
Respiratory Rate&
&
220210&
breaths per min\\
5&
O2 saturation pulseoxymetry&
&
220277&
percent\\
6&
Arterial BP [Systolic]&
&
51&
mmhg\\
7&
Arterial BP [Diastolic]&
&
8368&
mmhg\\
8&
Arterial BP Mean&
&
52&
mmhg\\
9&
Urine Out Foley&
&
40055&
ml\\
10&
HR Alarm [High]&
&
8549&
bpm\\
11&
HR Alarm [Low]&
&
5815&
bpm\\
12&
SpO2 Alarm [Low]&
&
5820&
percent\\
13&
SpO2 Alarm [High]&
&
8554&
percent\\
14&
Resp Alarm [High]&
&
8553&
bpm\\
15&
Resp Alarm [Low]&
&
5819&
bpm\\
16&
SaO2&
&
834&
percent\\
17&
HR Alarm [Low]&
&
3450&
bpm\\
18&
HR Alarm [High]&
&
8518&
bpm\\
19&
Resp Rate&
&
3603&
breaths\\
20&
SaO2 Alarm [Low]&
&
3609&
cm h2o\\
21&
SaO2 Alarm [High]&
&
8532&
cm h2o\\
22&
Previous WeightF&
&
581&
kg\\
23&
NBP [Systolic]&
&
455&
mmhg\\
24&
NBP [Diastolic]&
&
8441&
mmhg\\
25&
NBP Mean&
&
456&
mmhg\\
26&
NBP Alarm [Low]&
&
5817&
mmhg\\
27&
NBP Alarm [High]&
&
8551&
mmhg\\
28&
Non Invasive Blood Pressure mean&
&
220181&
mmhg\\
29&
Non Invasive Blood Pressure systolic&
&
220179&
mmhg\\
30&
Non Invasive Blood Pressure diastolic&
&
220180&
mmhg\\
31&
Foley&
&
226559&
ml\\
32&
CVP&
&
113&
mmhg\\
33&
Arterial Blood Pressure mean&
&
220052&
mmhg\\
34&
Arterial Blood Pressure systolic&
&
220050&
mmhg\\
35&
Arterial Blood Pressure diastolic&
&
220051&
mmhg\\
36&
ABP Alarm [Low]&
&
5813&
mmhg\\
37&
ABP Alarm [High]&
&
8547&
mmhg\\
38&
GCS Total&
&
198&
missing\\
39&
Hematocrit&
4544-3&
&
percent\\
40&
Potassium&
2823-3&
&
meq per l\\
41&
Hemoglobin [Mass/volume] in Blood&
718-7&
&
g per dl\\
42&
Sodium&
2951-2&
&
meq per l\\
43&
Creatinine&
2160-0&
&
mg per dl\\
44&
Chloride&
2075-0&
&
meq per l\\
45&
Urea Nitrogen&
3094-0&
&
mg per dl\\
46&
Bicarbonate&
1963-8&
&
meq per l\\
47&
Platelet Count&
777-3&
&
k per ul\\
48&
Anion Gap&
1863-0&
&
meq per l\\
49&
Temperature F&
&
678&
deg f\\
50&
Temperature C (calc)&
&
677&
deg f\\
51&
Leukocytes [\#/volume] in Blood by Manual count&
804-5&
&
k per ul\\
52&
Glucose&
2345-7&
&
mg per dl\\
53&
Erythrocyte mean corpuscular hemoglobin concentration [Mass/volume] by Automated count&
786-4&
&
percent\\
54&
Erythrocyte mean corpuscular hemoglobin [Entitic mass] by Automated count&
785-6&
&
pg\\
55&
Erythrocytes [\#/volume] in Blood by Automated count&
789-8&
&
per nl\\
56&
Erythrocyte mean corpuscular volume [Entitic volume] by Automated count&
787-2&
&
fl\\
57&
Erythrocyte distribution width [Ratio] by Automated count&
788-0&
&
percent\\
58&
Temp/Iso/Warmer [Temperature degrees C]&
&
8537&
deg f\\
59&
FIO2&
&
3420&
percent\\
60&
Magnesium&
2601-3&
&
mg per dl\\
61&
CVP Alarm [High]&
&
8548&
mmhg\\
62&
CVP Alarm [Low]&
&
5814&
mmhg\\
63&
Calcium [Moles/volume] in Serum or Plasma&
2000-8&
&
mg per dl\\
64&
Phosphate&
2777-1&
&
mg per dl\\
65&
FiO2 Set&
&
190&
torr\\
66&
Temp Skin [C]&
&
3655&
in\\
67&
pH&
11558-4&
&
u\\
68&
Temperature Fahrenheit&
&
223761&
deg f\\
69&
Central Venous Pressure&
&
220074&
mmhg\\
70&
Inspired O2 Fraction&
&
223835&
percent\\
71&
PAP [Systolic]&
&
492&
mmhg\\
72&
PAP [Diastolic]&
&
8448&
mmhg\\
73&
Calculated Total CO2&
34728-6&
&
meq per l\\
74&
Oxygen [Partial pressure] in Blood&
11556-8&
&
mmhg\\
75&
Base Excess&
11555-0&
&
meq per l\\
76&
Carbon dioxide [Partial pressure] in Blood&
11557-6&
&
mmhg\\
77&
PTT&
3173-2&
&
s\\
78&
Deprecated INR in Platelet poor plasma by Coagulation assay&
5895-7&
&
ratio\\
79&
PT&
5902-2&
&
s\\
80&
Temp Axillary [F]&
&
3652&
deg f\\
81&
Day of Life&
&
3386&
\\
82&
Total Fluids cc/kg/d&
&
3664&
\\
83&
Present Weight (kg)&
&
3580&
kg\\
84&
Present Weight (lb)&
&
3581&
cm h2o\\
85&
Present Weight (oz)&
&
3582&
cm h2o\\
86&
Fingerstick Glucose&
&
807&
mg per dl\\
87&
PEEP set&
&
220339&
cm h2o\\
88&
Previous Weight (kg)&
&
3583&
kg\\
89&
Weight Change (gms)&
&
3692&
g\\
90&
PEEP Set&
&
506&
cm h2o\\
91&
Mean Airway Pressure&
&
224697&
cm h2o\\
92&
Tidal Volume (observed)&
&
224685&
ml\\
93&
Resp Rate (Total)&
&
615&
bpm\\
94&
Minute Volume Alarm - High&
&
220293&
l per min\\
95&
Minute Volume Alarm - Low&
&
220292&
l per min\\
96&
Apnea Interval&
&
223876&
s\\
97&
Minute Volume&
&
224687&
l per min\\
98&
Paw High&
&
223873&
cm h2o\\
99&
Peak Insp. Pressure&
&
224695&
cm h2o
\end{longtabu}

\section{Additional Experiment Results}

\begin{table}[h!]
\centering
\begin{center}
\begin{tabular}{c  p{1.8cm}   p{1.8cm} p{1.8cm}   p{1.8cm}   p{1.8cm}}  \\
\toprule 
                & C-Index& AUC-ROC@24 & AP@24 & AUC-ROC@48 &  AP@48 \\
 \hline
Deep Cox     &  0.771 [0.750, 0.814] &0.835 [0.782, 0.901] & 0.094 [0.047, 0.185] & 0.828 [0.793, 0.858] & 0.106 [0.065, 0.183]  \\ 
 \hline                 
LSTM + Exp  & 0.790      [0.746, 0.819] & 0.851 [0.777, 0.909] & 0.260 [0.126, 0.425] & 0.835 [0.760, 0.905] & 0.262 [0.154, 0.372]\\ 
 \hline                 
LSTM + State    & 0.799  [0.769, 0.841]& 0.890 [0.835, 0.934] & 0.313 [0.220, 0.470] & 0.867 [0.800, 0.927] & 0.362 [0.260, 0.498] \\ 
 \hline 
DSSM + Exp     & 0.797 [0.758, 0.820] & 0.883 [0.836, 0.930] & 0.298 [0.165, 0.474] & 0.875 [0.830, 0.922] &   0.309 [0.164, 0.450]\\ 
 \hline 
DSSM + State    & \textbf{0.809} [0.775, 0.831] & \textbf{0.896} [0.834, 0.955] & \textbf{0.357} [0.169, 0.553] & \textbf{0.881} [0.837, 0.908] & \textbf{0.365} [0.280, 0.452] \\ 
 \bottomrule
\end{tabular}
\end{center}
\caption{Time-to-Mortality Prediction Results.}
\label{table:survival_result}
\end{table}


==> discussion.tex <==
\section{Discussion Note}

\subsection{03/26}
\begin{itemize}
    \item Denny: Focus on healthcare app task. One of the contributions is the new ML task in healthcare domain. 
\end{itemize}

\subsection{03/22}
\begin{itemize}
    \item Loss function for system identification. x has two components -- mask and value. how to define loss?
    \item intervention embedding layer to reduce dimension.
    \item Denny: use RNN directly, plot a new RNN architecture. 
\end{itemize}

\subsection{03/21}
\begin{itemize}
    \item Denny: Use a NN for generation more flexible distribution.
    \item Denny/Kun: observation sampling and mask. x can be a deterministic function of s and a.
    \item Nan: prediction task and relationship with marked point process: Do not mention point process as people will ask about hazard rate. We just do prediction of event mark/value at a given time point.
    \item Kun: Intervention dimension can be too large for mimic. We need to encode it to a low dimension as well. For forecasting, we only need the low-dimension encoding of intervention.
\end{itemize}

\section{Progress}

\begin{itemize}
\item RNN2-LSTM (with separation of intervention and feature).
- data format/provider change
- synthetic data gen.
- 

\item Prediction data set (mortality): link to spreadsheet


\item LSTM baseline


\item RNN2-LSTM with sampling model
\item RNN2-LSTM with intervention forecast

\end{itemize}



\begin{figure}\centering
% 	\begin{tikzpicture}
%         \draw (0,0) -- (0,5);
%         \draw (0,0.5) -- (5,0.5); 
%         \node [right] at (5, 0.5) {E}; 
%         \draw (0,1.5) -- (8,1.5); 
%         \draw [fill] (8, 1.5) circle [radius=0.2]; 
%         \draw (0,2.5) -- (2,2.5); 
%         \node [right] at (2, 2.5) {E}; 
%         \draw (0,3.5) -- (3,3.5); 
%         \draw [fill] (3,3.5) circle [radius=0.2]; 
%         \draw (0, 4.5) -- (6, 4.5); 
%         \node [right] at (6,4.5) {E}; 
%         \draw (8,0) -- (8,5);
%         \node [left] at (-0.5, 4.5) {1}; 
%         \node [left] at (-0.5, 3.5) {2}; 
%         \node [left] at (-0.5, 2.5) {3};
%         \node [left] at (-0.5, 1.5) {4};
%         \node [left] at (-0.5, 0.5) {5};
%          \node at (0, -0.8) {Start}; 
%          \node at (8, -0.8) {End}; 
% 	\end{tikzpicture}
\scalebox{.8}{
    	\begin{tikzpicture}
        \draw (0,0) -- (0,5);
        \draw[->] (0,0.5) -- (5,0.5); 
        \node [right] at (5, 0.5) {Event}; 
        \draw[->] (0,1.5) -- (8,1.5); 
        \draw[->] (0,2.5) -- (2,2.5); 
        \node [right] at (2, 2.5) {Event}; 
        \draw[->] (0,3.5) -- (3,3.5); 
        \node [right] at (3, 3.5) {Drop out}; 
        \draw[->] (0, 4.5) -- (6, 4.5); 
        \node [right] at (6,4.5) {Event }; 
        \draw (8,0) -- (8,5);
        \node [left] at (-0.5, 4.5) {A}; 
        \node [left] at (-0.5, 3.5) {B}; 
        \node [left] at (-0.5, 2.5) {C};
        \node [left] at (-0.5, 1.5) {D};
        \node [left] at (-0.5, 0.5) {E};
         \node at (0, -0.5) {Start}; 
         \node at (8, -0.5) {End}; 
	\end{tikzpicture}
	}
    \caption{Illustration of censored data. Of the five persons, three get the event (person A,  C and E), and two are censored (person B and D). Person B and D have different censoring types.  Person B drops out of the study, while person D have not experienced the event till the end of  the study.}
	\label{fig:time2event}
\end{figure}



==> extension.tex <==
\section{Model Extensions}

\subsection{Multi-Scale System Model}

The basic system model assumes that the entire population share the same dynamic physiological system. In reality, different sub-population groups may exhibit different dynamic behaviors. To address this issue, we encode the static context features such as age, gender, admission diagnosis using a NN to form the initial state for the LGSS. \footnote{another option is to use this vector to modulate the transition matrix, emission matrix. Are they essentially the same effort?}.


\subsection{Nonlinear System}

Replace the linear transitions with NN. Several existing works have already done so. Our method works with any one.






==> related.tex <==
\section{Related Works}

These are three main areas of work upon which this paper builds:

\textbf{Clinical prediction}. Deep learning models are increasingly used to improve the predictions of clinical outcomes such as mortality or diagnosis~\cite{rajkomar18scalable, bcb2017-sha, Che2018-vj, Choi2015-ak, iclr16-lipton}. These works can be roughly categorized based on the data, models and the prediction tasks used. Our work uses clinical time-series data, similar to ~\cite{aaai2018-song, aim2013-liu, aaai2016-liu, iclr16-lipton, jaim2017-wu} to make predictions. Our work is related to the switching discrete state space models of \cite{ghassemi-switching}, which was used to predict clinical interventions in ICU, and the continuous state space model o\cite{pmlr-v68-raghu17a}, which learns a treatment policy using deep reinforcement learning. However, our task, providing a joint forecast of the trajectory of observations and interventions, has not been considered by these previous works.


\textbf{Deep state space model}. A few recent works~\cite{nipsw15-dkf, aaai17-sontag-dmm, iclr17-dvbf, nips17-marco-kvae, nips16-marco-srnn} have extended the traditional linear Gaussian state space model to handle non-linear relations via neural networks. The goal of these works is to fit a generative model to a sequence of observations and actions, while ours is to capture the inherent state transition dynamics and use it for forecasting. From this perspective, our work is related to the work of~\citet{nips18-amazon} which combines a state space model with deep learning for time-series forecasting. Our differences lie in two aspects: 1) in \cite{nips18-amazon}, it is assumed that the co-variants are available in the forecast horizon; we do not make this assumption -- instead we provide joint intervention forecasting; 2) The training loss in ~\cite{nips18-amazon} is based on the data likelihood from the history while the same state transition function is applied and rolled out for prediction. In our work, the model is pretrained based on the entire trajectory of the patient records and fine tuned based on the data likelihood in the predicted horizon.
